Tropical geometry

Tropical mathematics redefines the rules of arithmetic by replacing addition with taking a maximum, and by replacing multiplication with addition. After briefly discussing a tropical version of linear algebra, we study polynomials build with these new operations. These equations define piecewise-linear geometric objects called tropical varieties. We explore these tropical varieties in two and three dimensions, building up discrete tools for studying them and determining their geometric properties. We then discuss the relationship between tropical geometry and algebraic geometry, which considers shapes defined by usual polynomial equations.

==> Ralph Morrison Chapter/referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 

\bibitem{amm}  Amdeberhan, T., Medina, L. A., Moll, V. H.: Asymptotic valuations of sequences satisfying first order recurrences. Proc. Amer. Math. Soc. \textbf{137},  no. 3 (2009)


\bibitem{blmpr}  Baker, M., Len, Y., Morrison, R.,  Pflueger, N.,  Ren, Q.: Bitangents of tropical plane quartic curves. Math. Z. \textbf{282}, no. 3-4 (2016)

\bibitem{baker-norine} Baker, M., Norine, S.: Riemann-Roch and Abel-Jacobi theory on a finite graph. Adv. Math. 215 no. 2 (2007)

\bibitem{balaban} Balaban, A.T.: Enumeration of cyclic graphs.  Chemical Applications of Graph Theory (A.T. Balaban, ed.) 63?105, Academic Press (1976)

\bibitem{bkt} Bashelor, A., Ksir, A., Traves, W.: Enumerative algebraic geometry of conics. Amer. Math. Monthly \textbf{115}, no. 8  (2008)

\bibitem{bmv} Brannetti, S., Melo, M., Viviani, F.: On the tropical Torelli map. Adv. Math.,
226(3) (2011)

\bibitem{bjms} Brodsky, S., Joswig, M., Morrison, R. Sturmfels, B.: Moduli of tropical plane curves. Res. Math. Sci. \textbf{2}, Art. 4 (2015)

\bibitem{butkovic} Butkovi\u c, P.:  Max-linear systems: theory and algorithms. Springer Monographs in Mathematics. Springer-Verlag London, Ltd., London (2010). 

\bibitem{sprawling}Cartwright, D., Dudzik, A., Manjunath, M., Yao, Y.: Embeddings and immersions of tropical curves. Collect. Math. \textbf{67}, no. 1 (2016)

\bibitem{movingout} Castryck, W.: Moving out the edges of a lattice polygon. Discrete and Computational Geometry \textbf{47}, no. 3 (2012)

\bibitem{cv} Castryck, W., Voight, J.: On nondegeneracy of curves. Algebra and Number Theory \textbf{3} (2009)

\bibitem{chan} Chan, M.: Combinatorics of the tropical Torelli map. Algebra Number Theory,
6(6) (2012)

\bibitem{chan2}  Chan, M.: Tropical hyperelliptic curves. J. Algebraic Combin. \textbf{37}, no. 2 (2013)

\bibitem{k4}  Chan, M., Jiradilok, P.: Theta characteristics of tropical $K_4$-curves. Combinatorial algebraic geometry, 65--86, Fields Inst. Commun., 80, Fields Inst. Res. Math. Sci., Toronto, ON (2017)

\bibitem{cd}  Cools, F., Draisma, J.: On metric graphs with prescribed gonality. J. Combin. Theory Ser. A \textbf{156} (2018)

\bibitem{chip-firing} Corry, S., Perkinson, D: Divisors and sandpiles. An introduction to chip-firing. American Mathematical Society, Providence, RI (2018)



\bibitem{clo} Cox, D. A., Little, J., O'Shea, D.: Ideals, varieties, and algorithms. An introduction to computational algebraic geometry and commutative algebra. Fourth edition. Undergraduate Texts in Mathematics. Springer, Cham, xvi+646 pp. (2015)

\bibitem{de} de Bruijn, N. G., Erdös, P: On a combinatorial problem. Nederl. Akad. Wetensch., Proc. \textbf{51} (1948) 

\bibitem{triangulations}  De Loera, J.A., Rambau, J., Santos, F.: Triangulations. Structures for algorithms and applications. Algorithms and Computation in Mathematics, 25. Springer-Verlag, Berlin (2010)

\bibitem{sevencircles}  Evelyn, C. J. A., Money-Coutts, G. B.,Tyrrell, J. A.: The seven circles theorem and other new theorems. Stacey International, London (1974)

\bibitem{fno}  Farouki, R.T., Neff, C., O'Conner, M.A.:  Automatic parsing of degenerate quadric-surface intersections.  ACM Transactions on Graphics (TOG) \textbf{8}, No. 3 (1989)

\bibitem{gk}  Gathmann, A., Kerber, M.: A Riemann-Roch theorem in tropical geometry. Math. Z. \textbf{259}, no. 1 (2008)

\bibitem{polymake}   Gawrilow, E., Joswig, M.: polymake: a framework for analyzing convex polytopes. Polytopes-combinatorics and computation (Oberwolfach, 1997), 43?73, DMV Sem., 29, Birkhäuser, Basel (2000)

\bibitem{tropicalschemes}  Giansiracusa, J., Giansiracusa, N.: Equations of tropical varieties. Duke Math. J. \textbf{165}, no. 18, 3379--3433 (2016)

\bibitem{m2} Grayson, D., Stillman, M. E.:  Macaulay2, a software system for research in algebraic geometry. Available at \url{http://www.math.uiuc.edu/Macaulay2/}



\bibitem{hmrt}  Hahn, M.A.,  Markwig, H.,  Ren, Y., Tyomkin, I.: Tropicalized quartics and canonical embeddings for tropical curves of genus 3. arXiv preprint \texttt{arXiv:1802.02440} (2018)



\bibitem{hartshorne}
Hartshorne, R.: Algebraic geometry. Graduate Texts in Mathematics, No. 52. Springer-Verlag, New York-Heidelberg {\rm xvi}+496 pp. (1977)

\bibitem{hilbert}
Hilbert, D.: Ueber die Theorie der algebraischen Formen. (German) Math. Ann. \textbf{36},  no. 4 (1890)

\bibitem{gfan}   Jensen, A.: Gfan, a software system for Gr\"{o}bner fans and tropical varieties. Available at
\url{http://home.imf.au.dk/jensen/software/gfan/gfan.html}.

\bibitem{kz} Kaibel, V., Ziegler, G.M.: Counting lattice triangulations. Surveys in combinatorics, 2003 (Bangor), 277--307, London Math. Soc. Lecture Note Ser., 307, Cambridge Univ. Press, Cambridge, (2003)

\bibitem{koelman}   Koelman, R.: The number of moduli of families of curves on toric surfaces.
Ph.D. thesis, Katholieke Universiteit Nijmegen (1991)

\bibitem{lz}  Lagarias, J.C., Ziegler,  G.M.: Bounds for lattice polytopes containing a fixed number of
interior points in a sublattice. Canadian J. Math. \textbf{43} (1991)

\bibitem{legall} Le Gall, François: Powers of tensors and fast matrix multiplication. Proceedings of the 39th International Symposium on Symbolic and Algebraic Computation (ISSAC 2014)



\bibitem{lifting}  Len, Y., Markwig, H..: Lifting tropical bitangents. arXiv preprint \texttt{arXiv:1708.04480} (2018)

\bibitem{lifting-self}  Len, Y., Satriano., M.: Lifting tropical self intersections. arXiv preprint \texttt{arXiv:1806.01334} (2018)


\bibitem{lengyel} Lengyel, T.: On the divisibility by $2$ of the Stirling numbers of the second kind. Fibonacci Quart. \textbf{32}, no. 3 (1994)


\bibitem{lin-tran}  Lin, B., Tran, N. M.: Linear and rational factorization of tropical polynomials. arXiv preprint \texttt{arXiv:1707.03332} (2017)

\bibitem{tropicalideals} Maclagan, D., Rinc\'{o}n, F.: Tropical ideals. Compos. Math. \textbf{154}, no. 3   (2018)

\bibitem{maclagan-sturmfels}  Maclagan, D., Sturmfels, B.: Introduction to tropical geometry. Graduate Studies in Mathematics, 161. American Mathematical Society, Providence, RI (2015)

\bibitem{fibonacci}  Medina, L. A., Rowland, E.: $p$-regularity of the $p$-adic valuation of the Fibonacci sequence. Fibonacci Quart. \textbf{53}, no. 3 (2015)

\bibitem{mz}  Mikhalkin, G., Zharkov, I.: Tropical curves, their Jacobians and theta functions. Curves and abelian varieties, 203--230, Contemp. Math., 465, Amer. Math. Soc., Providence, RI (2008)


\bibitem{morrison-hyperelliptic}  Morrison, R.: Tropical hyperelliptic curves in the plane. arXiv preprint \texttt{arXiv:1708.00571} (2017)

\bibitem{tropical-images}  Morrison, R: Tropical images of intersection points. Collect. Math. \textbf{66}, no. 2 (2015)


\bibitem{op} Osserman, B., Payne, S.: Lifting tropical intersections. Doc. Math. \textbf{18} (2013)

\bibitem{or}  Osserman, B., Rabinoff, J.: Lifting nonproper tropical intersections. Tropical and non-Archimedean geometry, 15--44, Contemp. Math., 605, Centre Rech. Math. Proc., Amer. Math. Soc., Providence, RI, (2013)


\bibitem{pick} Pick, G. A.:  Geometrisches zur Zahlenlehre, Sitzenber. Lotos (Prague) \textbf{19} (1899)

\bibitem{pin} Pin, J.: Tropical semirings. Idempotency (Bristol, 1994), 50--69, Publ. Newton Inst., 11, Cambridge Univ. Press, Cambridge (1998)


\bibitem{plucker}  Pl\"{u}cker, J.: Solution d'une question fondamentale concernant la théorie générale des courbes. (French) J. Reine Angew. Math. \textbf{12} (1834)


\bibitem{firststeps}  Richter-Gebert, J., Sturmfels, B., Theobald, T.: First steps in tropical geometry. Idempotent mathematics and mathematical physics, 289--317, Contemp. Math., \textbf{377}, Amer. Math. Soc., Providence, RI (2005)

\bibitem{topcom} Rambau, J.: TOPCOM: Triangulations of Point Configurations and Oriented Matroids, Mathematical Software - ICMS 2002 (Cohen, Arjeh M. and Gao, Xiao-Shan and Takayama, Nobuki, eds.), World Scientific, pp. 330-340 (2002)

\bibitem{scott}  Scott, P.R.: On convex lattice polygons. Bull. Austral. Math. Soc. \textbf{15} (1976)

\bibitem{simon}  Simon, I.: Recognizable sets with multiplicities in the tropical semiring. Mathematical foundations of computer science, 1988 (Carlsbad, 1988), 107--120, Lecture Notes in Comput. Sci., 324, Springer, Berlin, (1988)

\bibitem{strassen}  Strassen, V.: Gaussian Elimination is not Optimal. Numer. Math. \textbf{13} (1969)

\end{thebibliography}

